3SAT on an All-to-All-Connected CMOS Ising Solver Chip

This work solves 3SAT, a classical NP-complete problem, on a CMOS-based Ising hardware chip with all-to-all connectivity. The paper addresses practical issues in going from algorithms to hardware. It considers several degrees of freedom in mapping the 3SAT problem to the chip - using multiple Ising formulations for 3SAT; exploring multiple strategies for decomposing large problems into subproblems that can be accommodated on the Ising chip; and executing a sequence of these subproblems on CMOS hardware to obtain the solution to the larger problem. These are evaluated within a software framework, and the results are used to identify the most promising formulations and decomposition techniques. These best approaches are then mapped to the all-to-all hardware, and the performance of 3SAT is evaluated on the chip. Experimental data shows that the deployed decomposition and mapping strategies impact SAT solution quality: without our methods, the CMOS hardware cannot achieve 3SAT solutions on SATLIB benchmarks.

==> figtbls/chip.tex <==
\begin{table}[t]
    \caption{Specifications of the CMOS Ising chip.}
    \label{tab:chip_spec}
    \centering
    \begin{tabular}{|l|l|}
        \hline Technology               & TSMC 65nm \\
        \hline Topology                 & All-to-all \\
        \hline Spin count               & 49 \\
        \hline Weights $\left( J_{ij}, h_i \right)$ 
                                        & $\{-14, \cdots, +14\}$~(29 levels) \\
        \hline Maximum power            & 0.12W @1.3V \\
        \hline Ising core area          & 0.28mm$^2$ \\
        \hline Oscillation frequency    & 26MHz \\
        \hline Relaxation time          & 40~cycles \\
        \hline
    \end{tabular}
\vspace{-6mm}
\end{table}

==> figtbls/obsolete_uf20-01_mapping.tex <==
% \begin{figure}[tb]
%     \centering
%     % \begin{subfigure}[]{}
%     \subfloat[]{
%         \begin{tikzpicture}
%         \begin{axis}[
%             axis line style={draw=none},
%             tick style={draw=none},
%             axis background/.style={fill=gray!5},
%             width=.45\columnwidth,
%             height=.45\columnwidth,
%             grid=both, 
%             grid style={white},
%             legend cell align={left},
%             legend entries={Chip,Software},
%             legend style={fill==gray!10, fill opacity=0.6, draw opacity=1, text opacity=1, draw=gray!20},
%             legend pos=south west,
%             xlabel={Subproblem number},
%             ylabel={Energy},
%             enlargelimits=false,
%         ]
%             \addplot +[mark=none] table {data/subproblem_accuracy_ground/chip_uf20-01-scale12-size47lfsize2.dat}; 
%             \addplot +[mark=none] table {data/subproblem_accuracy_ground/qbsolv_uf20-01-scale12-size47lfsize2.dat}; 
%         \end{axis}
%         \end{tikzpicture}
%     }
%     % \end{subfigure}
%     % \begin{subfigure}[]{}
%     \subfloat[]{
%         \begin{tikzpicture}
%         \begin{axis}[
%             axis line style={draw=none},
%             tick style={draw=none},
%             axis background/.style={fill=gray!5},
%             width=.45\columnwidth,
%             height=.45\columnwidth,
%             grid=both, 
%             grid style={white},
%             legend cell align={left},
%             legend entries={Chip,Software},
%             legend style={fill==gray!10, fill opacity=0.6, draw opacity=1, text opacity=1, draw=gray!20},
%             legend pos=south west,
%             xlabel={Subproblem number},
%             ylabel={Energy},
%             enlargelimits=false,
%         ]
%             \addplot +[mark=none] table {data/subproblem_accuracy_ground/chip_uf20-01-scale12-size39lfsize10.dat}; 
%             \addplot +[mark=none] table {data/subproblem_accuracy_ground/qbsolv_uf20-01-scale12-size39lfsize10.dat}; 
%         \end{axis}
%         \end{tikzpicture}
%     }
%     % \end{subfigure}
%     \caption{uf20-01 subproblem software and chip energies with (a) 2-LFROSC (b) 10-LFROSC when the scaling factor is 12.\redHL{Too much white space around the figure; legends overlap the figure making it hard to view; caption too long, inconsistent with other captions: let us describe the conclusions of the figure in the text rather than in the caption.}\husrev{Will work on the whitespace\&legend, all the information in the caption is in the main text so I pruned it.}}
%     \label{fig:subproblem_ground_lfrosc}
% \end{figure}
